Single-View Rolling-Shutter SfM

Rolling-shutter (RS) cameras are ubiquitous, but RS SfM (structure-from-motion) has not been fully solved yet. This work suggests an approach to remedy this: We characterize RS single-view geometry of observed world points or lines. Exploiting this geometry, we describe which motion and scene parameters can be recovered from a single RS image and systematically derive minimal reconstruction problems. We evaluate several representative cases with proof-of-concept solvers, highlighting both feasibility and practical limitations.

==> Plot/noise_r_angle.tex <==
\begin{axis}[%
xmode=log,
width=0.16\columnwidth,
height=0.10\columnwidth,
at={(3.15in,0.389in)},
scale only axis,
xmin=0.01,
xmax=5,
xlabel style={font=\color{white!15!black}},
xlabel={Norm err (rel.)},
ymin=0,
ymax=1,
%ytick={0,10000},
%xtick={1e-6,1e-15},
ytick={0,0.5,1},
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=VeryPink,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
0.0131826 0.00639\\
0.0229087 0.01083\\
0.0398107 0.01865\\
0.0691831 0.03119\\
0.120226 0.05077\\
0.20893 0.082\\
0.363078 0.12314\\
0.630957 0.18392\\
1.09648 0.38563\\
1.90546 0.91889\\
3.31131 0.97754\\
5.7544 0.9928\\
10 0.9974\\
17.378 0.99899\\
30.1995 0.99945\\
52.4807 0.99988\\
91.2011 0.99997\\
158.489 1\\
275.423 1\\
478.63 1\\
831.764 1\\
1445.44 1\\
2511.89 1\\
4365.16 1\\
7585.78 1\\
};
\addlegendentry{$\delta1p3$}

\addplot [color=brown,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
0.0131826 0.00133\\
0.0229087 0.0023\\
0.0398107 0.0037\\
0.0691831 0.00643\\
0.120226 0.01113\\
0.20893 0.01948\\
0.363078 0.03364\\
0.630957 0.06734\\
1.09648 0.25511\\
1.90546 0.88771\\
3.31131 0.96941\\
5.7544 0.98647\\
10 0.9911\\
17.378 0.99315\\
30.1995 0.99465\\
52.4807 0.99666\\
91.2011 0.99761\\
158.489 0.99849\\
275.423 0.999\\
478.63 0.99945\\
831.764 0.99963\\
1445.44 0.99986\\
2511.89 0.99994\\
4365.16 0.99997\\
7585.78 1\\
};
\addlegendentry{$\delta1p4$}

\addplot [color=cyan,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
0.0131826 8e-05\\
0.0229087 0.00015\\
0.0398107 0.00026\\
0.0691831 0.00048\\
0.120226 0.00071\\
0.20893 0.00141\\
0.363078 0.00304\\
0.630957 0.00831\\
1.09648 0.07333\\
1.90546 0.88782\\
3.31131 0.99318\\
5.7544 0.99765\\
10 0.99884\\
17.378 0.99908\\
30.1995 0.9994\\
52.4807 0.9997\\
91.2011 0.99988\\
158.489 0.99996\\
275.423 0.99996\\
478.63 1\\
831.764 1\\
1445.44 1\\
2511.89 1\\
4365.16 1\\
7585.78 1\\
};
\addlegendentry{$\delta1p5$}

\addplot [color=black,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
0.0131826 0.00061\\
0.0229087 0.00118\\
0.0398107 0.00201\\
0.0691831 0.00333\\
0.120226 0.00594\\
0.20893 0.01018\\
0.363078 0.02036\\
0.630957 0.05236\\
1.09648 0.19892\\
1.90546 0.59633\\
3.31131 0.8718\\
5.7544 0.96867\\
10 0.99226\\
17.378 0.99756\\
30.1995 0.99924\\
52.4807 0.99981\\
91.2011 0.99991\\
158.489 0.99997\\
275.423 0.99999\\
478.63 1\\
831.764 1\\
1445.44 1\\
2511.89 1\\
4365.16 1\\
7585.78 1\\
};
\addlegendentry{$LAAA$}

\legend{}

\end{axis}

==> Plot/noise_t_line.tex <==
\begin{axis}[%
%xmode=log,
width=0.16\columnwidth,
height=0.10\columnwidth,
at={(1.05in,0.389in)},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black}},
xlabel={Line err ($^\circ$)},
ymin=0,
ymax=1,
%ytick={0,10000},
ytick={0,0.5,1},
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=red,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
1 0.03341\\
2 0.07072\\
3 0.1027\\
4 0.13004\\
5 0.1541\\
6 0.17552\\
7 0.19436\\
8 0.21092\\
9 0.22627\\
10 0.24011\\
11 0.25353\\
12 0.26588\\
13 0.27721\\
14 0.28764\\
15 0.29731\\
16 0.30702\\
17 0.31634\\
18 0.32477\\
19 0.33289\\
20 0.34097\\
21 0.34872\\
22 0.35641\\
23 0.3634\\
24 0.37091\\
25 0.37836\\
26 0.38588\\
27 0.39332\\
28 0.40032\\
29 0.40764\\
30 0.4146\\
31 0.42181\\
32 0.42847\\
33 0.4354\\
34 0.44238\\
35 0.44975\\
36 0.45755\\
37 0.46469\\
38 0.47253\\
39 0.47989\\
40 0.48711\\
41 0.49473\\
42 0.5029\\
43 0.5104\\
44 0.51818\\
45 0.52594\\
46 0.53428\\
47 0.54248\\
48 0.55144\\
49 0.56016\\
50 0.56911\\
51 0.57806\\
52 0.58716\\
53 0.59621\\
54 0.60539\\
55 0.61428\\
56 0.62319\\
57 0.63211\\
58 0.64153\\
59 0.65133\\
60 0.66095\\
61 0.67079\\
62 0.68067\\
63 0.69107\\
64 0.70117\\
65 0.71149\\
66 0.72171\\
67 0.73188\\
68 0.74324\\
69 0.7536\\
70 0.76426\\
71 0.77529\\
72 0.78606\\
73 0.79676\\
74 0.8084\\
75 0.81998\\
76 0.83117\\
77 0.84284\\
78 0.85451\\
79 0.86635\\
80 0.87769\\
81 0.88959\\
82 0.90154\\
83 0.91315\\
84 0.92609\\
85 0.93771\\
86 0.95011\\
87 0.96274\\
88 0.97446\\
89 0.98687\\
90 1\\
};
\addlegendentry{$d1p4P$}

\addplot [color=green,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
1 0.03609\\
2 0.07165\\
3 0.10155\\
4 0.12756\\
5 0.15053\\
6 0.17195\\
7 0.19179\\
8 0.21008\\
9 0.22653\\
10 0.24232\\
11 0.25703\\
12 0.27138\\
13 0.28434\\
14 0.29759\\
15 0.31039\\
16 0.32289\\
17 0.33478\\
18 0.34608\\
19 0.35717\\
20 0.36781\\
21 0.37824\\
22 0.38809\\
23 0.39769\\
24 0.40733\\
25 0.41708\\
26 0.42663\\
27 0.43578\\
28 0.44486\\
29 0.45405\\
30 0.46328\\
31 0.47192\\
32 0.48068\\
33 0.48868\\
34 0.49714\\
35 0.50541\\
36 0.5138\\
37 0.52221\\
38 0.5305\\
39 0.5388\\
40 0.54741\\
41 0.55604\\
42 0.56429\\
43 0.57244\\
44 0.58153\\
45 0.59006\\
46 0.59851\\
47 0.60653\\
48 0.61496\\
49 0.62393\\
50 0.63274\\
51 0.64084\\
52 0.64958\\
53 0.65769\\
54 0.66625\\
55 0.6744\\
56 0.68318\\
57 0.69175\\
58 0.69986\\
59 0.70856\\
60 0.71767\\
61 0.72665\\
62 0.73568\\
63 0.74422\\
64 0.75335\\
65 0.76282\\
66 0.77224\\
67 0.78164\\
68 0.79092\\
69 0.79967\\
70 0.809\\
71 0.81815\\
72 0.8273\\
73 0.83604\\
74 0.8454\\
75 0.85513\\
76 0.86441\\
77 0.87422\\
78 0.88439\\
79 0.89407\\
80 0.90344\\
81 0.91293\\
82 0.92221\\
83 0.93187\\
84 0.94141\\
85 0.95092\\
86 0.96087\\
87 0.97102\\
88 0.98046\\
89 0.99008\\
90 1\\
};
\addlegendentry{$d1p3P$}

\addplot [color=blue,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
1 0.03053\\
2 0.05744\\
3 0.07929\\
4 0.09741\\
5 0.11502\\
6 0.13071\\
7 0.14632\\
8 0.16087\\
9 0.17486\\
10 0.18805\\
11 0.20043\\
12 0.21267\\
13 0.22439\\
14 0.23538\\
15 0.24691\\
16 0.25749\\
17 0.26753\\
18 0.27805\\
19 0.28833\\
20 0.29813\\
21 0.30834\\
22 0.3181\\
23 0.32759\\
24 0.3368\\
25 0.34644\\
26 0.35568\\
27 0.36513\\
28 0.37402\\
29 0.38291\\
30 0.39174\\
31 0.40074\\
32 0.41003\\
33 0.41921\\
34 0.42784\\
35 0.43621\\
36 0.44504\\
37 0.4539\\
38 0.4625\\
39 0.47138\\
40 0.48021\\
41 0.489\\
42 0.49756\\
43 0.50623\\
44 0.51454\\
45 0.52282\\
46 0.53165\\
47 0.54075\\
48 0.54974\\
49 0.55852\\
50 0.56752\\
51 0.57635\\
52 0.5858\\
53 0.5953\\
54 0.60467\\
55 0.61473\\
56 0.62399\\
57 0.63387\\
58 0.64355\\
59 0.65316\\
60 0.66305\\
61 0.67246\\
62 0.68174\\
63 0.69168\\
64 0.70195\\
65 0.71231\\
66 0.72295\\
67 0.73368\\
68 0.74399\\
69 0.75421\\
70 0.76523\\
71 0.77633\\
72 0.787\\
73 0.79853\\
74 0.80973\\
75 0.82092\\
76 0.8335\\
77 0.84454\\
78 0.85625\\
79 0.86805\\
80 0.87947\\
81 0.89131\\
82 0.90362\\
83 0.91526\\
84 0.92725\\
85 0.93939\\
86 0.95155\\
87 0.9636\\
88 0.97581\\
89 0.98764\\
90 1\\
};
\addlegendentry{$d1p3PC$}

\addplot [color=magenta,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
1 0.02866\\
2 0.05177\\
3 0.06998\\
4 0.08723\\
5 0.10254\\
6 0.11704\\
7 0.13115\\
8 0.14474\\
9 0.15749\\
10 0.17004\\
11 0.18215\\
12 0.19382\\
13 0.20424\\
14 0.21448\\
15 0.22416\\
16 0.2347\\
17 0.24447\\
18 0.25376\\
19 0.26325\\
20 0.27265\\
21 0.28246\\
22 0.2917\\
23 0.30043\\
24 0.30973\\
25 0.31923\\
26 0.32854\\
27 0.33744\\
28 0.34705\\
29 0.35619\\
30 0.36605\\
31 0.37561\\
32 0.38488\\
33 0.39455\\
34 0.40398\\
35 0.41358\\
36 0.42312\\
37 0.4329\\
38 0.44266\\
39 0.4524\\
40 0.46199\\
41 0.47101\\
42 0.48146\\
43 0.49169\\
44 0.50155\\
45 0.51071\\
46 0.52009\\
47 0.53033\\
48 0.54026\\
49 0.55029\\
50 0.56034\\
51 0.57088\\
52 0.5808\\
53 0.59074\\
54 0.60158\\
55 0.61267\\
56 0.6233\\
57 0.63346\\
58 0.64393\\
59 0.65464\\
60 0.66533\\
61 0.67601\\
62 0.68615\\
63 0.69723\\
64 0.70788\\
65 0.71878\\
66 0.72966\\
67 0.74078\\
68 0.75233\\
69 0.76363\\
70 0.77463\\
71 0.78578\\
72 0.79683\\
73 0.80841\\
74 0.81984\\
75 0.83041\\
76 0.84126\\
77 0.85262\\
78 0.86418\\
79 0.87551\\
80 0.88693\\
81 0.89868\\
82 0.90961\\
83 0.92119\\
84 0.93224\\
85 0.944\\
86 0.95471\\
87 0.96577\\
88 0.97673\\
89 0.98824\\
90 1\\
};
\addlegendentry{$d1p2PC$}

\addplot [color=orange,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.28825e-20 0 \\
};
\addlegendentry{$d2p6$}

\addplot [color=gray,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
};
\addlegendentry{$d3p8$}

\legend{}

\end{axis}

\input{Plot/noise_r_axis.tex}

==> Plot/real_r_norm.tex <==
\begin{axis}[%
xmode=log,
width=0.16\columnwidth,
height=0.10\columnwidth,
at={(3.15in,0.389in)},
scale only axis,
xmin=0.01,
xmax=5,
xlabel style={font=\color{white!15!black}},
xlabel={Norm err (rel.)},
ymin=0,
ymax=1,
%ytick={0,10000},
%xtick={1e-6,1e-15},
ytick={0,0.5,1},
xlabel style={yshift=0.07in},
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=VeryPink,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0	0	\\
0.0285524052826707	0.0078740157480315	\\
0.04056565397699	0.015748031496063	\\
0.0842056878913391	0.0236220472440945	\\
0.0948718902198369	0.031496062992126	\\
0.102814955050417	0.0393700787401575	\\
0.108995559379393	0.047244094488189	\\
0.117205262809614	0.0551181102362205	\\
0.1524052054943	0.062992125984252	\\
0.15921234078491	0.0708661417322835	\\
0.188991750554614	0.078740157480315	\\
0.192307881014174	0.0866141732283465	\\
0.19303443644361	0.094488188976378	\\
0.223983689542221	0.102362204724409	\\
0.294580829958957	0.110236220472441	\\
0.303293403818473	0.118110236220472	\\
0.307707547967682	0.125984251968504	\\
0.309394755903146	0.133858267716535	\\
0.323838121579371	0.141732283464567	\\
0.325080849258995	0.149606299212598	\\
0.345519959350122	0.15748031496063	\\
0.38198620366195	0.165354330708661	\\
0.433976939161104	0.173228346456693	\\
0.468864799411706	0.181102362204724	\\
0.501546247149884	0.188976377952756	\\
0.534637004811113	0.196850393700787	\\
0.571615016152708	0.204724409448819	\\
0.588648738328092	0.21259842519685	\\
0.609145976057001	0.220472440944882	\\
0.623526182199535	0.228346456692913	\\
0.667569075509601	0.236220472440945	\\
0.694478766175612	0.244094488188976	\\
0.727577754607298	0.251968503937008	\\
0.742991190989102	0.259842519685039	\\
0.759018545975448	0.267716535433071	\\
0.768053810515683	0.275590551181102	\\
0.775834942880096	0.283464566929134	\\
0.831193818616314	0.291338582677165	\\
0.866426645993429	0.299212598425197	\\
0.899104996379666	0.307086614173228	\\
0.920217432437996	0.31496062992126	\\
0.948670381591692	0.322834645669291	\\
1.07824624131761	0.330708661417323	\\
1.10965970202797	0.338582677165354	\\
1.12874347957807	0.346456692913386	\\
1.14097120182235	0.354330708661417	\\
1.14326754360101	0.362204724409449	\\
1.17448037367872	0.37007874015748	\\
1.17626352450216	0.377952755905512	\\
1.22468387048712	0.385826771653543	\\
1.24184283791572	0.393700787401575	\\
1.2542165345143	0.401574803149606	\\
1.2806106069668	0.409448818897638	\\
1.28311128700828	0.417322834645669	\\
1.31373727265438	0.425196850393701	\\
1.36999452634775	0.433070866141732	\\
1.38718748024571	0.440944881889764	\\
1.40048469392597	0.448818897637795	\\
1.47028323679842	0.456692913385827	\\
1.48861675512868	0.464566929133858	\\
1.51171429063468	0.47244094488189	\\
1.52225012149928	0.480314960629921	\\
1.52784608199061	0.488188976377953	\\
1.56292155186319	0.496062992125984	\\
1.60609369528566	0.503937007874016	\\
1.60625234216832	0.511811023622047	\\
1.62941789992689	0.519685039370079	\\
1.6575365326561	0.52755905511811	\\
1.66242780576564	0.535433070866142	\\
1.71733999492965	0.543307086614173	\\
1.78234471594051	0.551181102362205	\\
1.7954399414025	0.559055118110236	\\
1.83971381835322	0.566929133858268	\\
1.89759526599966	0.574803149606299	\\
1.90580527095804	0.582677165354331	\\
1.9143062370943	0.590551181102362	\\
1.95184735888802	0.598425196850394	\\
1.96038251001426	0.606299212598425	\\
1.96428056845825	0.614173228346457	\\
2.10785982276219	0.622047244094488	\\
2.24991653574766	0.62992125984252	\\
2.25890357988006	0.637795275590551	\\
2.26641413050682	0.645669291338583	\\
2.43896029827177	0.653543307086614	\\
2.44396604076375	0.661417322834646	\\
2.48089233029761	0.669291338582677	\\
2.56478103804584	0.677165354330709	\\
2.569471711443	0.68503937007874	\\
2.64312016457107	0.692913385826772	\\
2.69087906687962	0.700787401574803	\\
2.73578599169795	0.708661417322835	\\
2.75551258425078	0.716535433070866	\\
2.82374664697536	0.724409448818898	\\
2.93151046410409	0.732283464566929	\\
2.9449545275583	0.740157480314961	\\
3.27102008635374	0.748031496062992	\\
3.37016068471251	0.755905511811024	\\
3.39045888479066	0.763779527559055	\\
3.43814782235668	0.771653543307087	\\
3.58057551431707	0.779527559055118	\\
3.60901920909857	0.78740157480315	\\
3.74321426231459	0.795275590551181	\\
999	0.803149606299213	\\
1000	0.811023622047244	\\
1001	0.818897637795276	\\
1002	0.826771653543307	\\
1003	0.834645669291339	\\
1004	0.84251968503937	\\
1005	0.850393700787402	\\
1006	0.858267716535433	\\
1007	0.866141732283465	\\
1008	0.874015748031496	\\
1009	0.881889763779528	\\
1010	0.889763779527559	\\
1011	0.897637795275591	\\
1012	0.905511811023622	\\
1013	0.913385826771654	\\
1014	0.921259842519685	\\
1015	0.929133858267717	\\
1016	0.937007874015748	\\
1017	0.94488188976378	\\
1018	0.952755905511811	\\
1019	0.960629921259843	\\
1020	0.968503937007874	\\
1021	0.976377952755906	\\
1022	0.984251968503937	\\
1023	0.992125984251969	\\
1024	1	\\
};
\addlegendentry{$\delta1p3$}

\addplot [color=brown,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0	0	\\
0.0047113000121877	0.0078740157480315	\\
0.00725493282551622	0.015748031496063	\\
0.0301083725763296	0.0236220472440945	\\
0.033000165400739	0.031496062992126	\\
0.0469945036076234	0.0393700787401575	\\
0.0563163129816334	0.047244094488189	\\
0.0737000536488134	0.0551181102362205	\\
0.0780334112288045	0.062992125984252	\\
0.0843995360141442	0.0708661417322835	\\
0.0844094011337995	0.078740157480315	\\
0.0934112225162656	0.0866141732283465	\\
0.101795685820393	0.094488188976378	\\
0.102137308895087	0.102362204724409	\\
0.120631464194705	0.110236220472441	\\
0.136491512980591	0.118110236220472	\\
0.151828167853963	0.125984251968504	\\
0.154204979452256	0.133858267716535	\\
0.161650051611889	0.141732283464567	\\
0.179880999197937	0.149606299212598	\\
0.18262270898791	0.15748031496063	\\
0.184957850864583	0.165354330708661	\\
0.187316634203045	0.173228346456693	\\
0.18778901787711	0.181102362204724	\\
0.236029113357574	0.188976377952756	\\
0.236128813745179	0.196850393700787	\\
0.23644369390154	0.204724409448819	\\
0.244242909172255	0.21259842519685	\\
0.273302202690539	0.220472440944882	\\
0.278763938036757	0.228346456692913	\\
0.290807914403988	0.236220472440945	\\
0.296599217499401	0.244094488188976	\\
0.297403705391506	0.251968503937008	\\
0.32701487041307	0.259842519685039	\\
0.333999883142076	0.267716535433071	\\
0.334679152739502	0.275590551181102	\\
0.345048510750424	0.283464566929134	\\
0.346381710207498	0.291338582677165	\\
0.352088516353507	0.299212598425197	\\
0.359188814283589	0.307086614173228	\\
0.365121358388335	0.31496062992126	\\
0.37124579069667	0.322834645669291	\\
0.372134966989191	0.330708661417323	\\
0.380325270178486	0.338582677165354	\\
0.384109762136177	0.346456692913386	\\
0.387386987351043	0.354330708661417	\\
0.396346666837418	0.362204724409449	\\
0.3999589900627	0.37007874015748	\\
0.403848840664214	0.377952755905512	\\
0.405327035098111	0.385826771653543	\\
0.407237288572356	0.393700787401575	\\
0.420868800602212	0.401574803149606	\\
0.435145535937698	0.409448818897638	\\
0.452615791533542	0.417322834645669	\\
0.469850568185626	0.425196850393701	\\
0.49547907270255	0.433070866141732	\\
0.497933002349864	0.440944881889764	\\
0.507201939874764	0.448818897637795	\\
0.507225669433649	0.456692913385827	\\
0.522493277213892	0.464566929133858	\\
0.571882789522954	0.47244094488189	\\
0.58412774873727	0.480314960629921	\\
0.586526103615112	0.488188976377953	\\
0.597214547823087	0.496062992125984	\\
0.601249763177288	0.503937007874016	\\
0.621627719984862	0.511811023622047	\\
0.623900498887901	0.519685039370079	\\
0.654154779969667	0.52755905511811	\\
0.672580985998231	0.535433070866142	\\
0.681574942297893	0.543307086614173	\\
0.682582911355859	0.551181102362205	\\
0.685466504863359	0.559055118110236	\\
0.687335322370974	0.566929133858268	\\
0.697988291629372	0.574803149606299	\\
0.69945622256583	0.582677165354331	\\
0.737690877621817	0.590551181102362	\\
0.738775932233122	0.598425196850394	\\
0.743346793525127	0.606299212598425	\\
0.744359103966256	0.614173228346457	\\
0.810222066681248	0.622047244094488	\\
0.830349980698061	0.62992125984252	\\
0.835496349596343	0.637795275590551	\\
0.84073921649984	0.645669291338583	\\
0.846406011654761	0.653543307086614	\\
0.885791594900921	0.661417322834646	\\
0.895593629567074	0.669291338582677	\\
0.900485944755931	0.677165354330709	\\
0.902703606081816	0.68503937007874	\\
0.906122820810126	0.692913385826772	\\
0.917744257865387	0.700787401574803	\\
0.935183570765325	0.708661417322835	\\
0.945429396901349	0.716535433070866	\\
1.00668098261806	0.724409448818898	\\
1.10210906632211	0.732283464566929	\\
1.10459176561783	0.740157480314961	\\
1.11706617485142	0.748031496062992	\\
1.11865005594733	0.755905511811024	\\
1.16286676489185	0.763779527559055	\\
1.17393577486314	0.771653543307087	\\
1.18429507433227	0.779527559055118	\\
1.19082958741894	0.78740157480315	\\
1.23302807959779	0.795275590551181	\\
1.24640817900832	0.803149606299213	\\
1.24917874499808	0.811023622047244	\\
1.2548129775274	0.818897637795276	\\
1.42967317580733	0.826771653543307	\\
1.43468367044801	0.834645669291339	\\
1.45636730158335	0.84251968503937	\\
1.46073363153776	0.850393700787402	\\
1.4723472199743	0.858267716535433	\\
1.49048295484354	0.866141732283465	\\
1.52048608996648	0.874015748031496	\\
1.53858179187891	0.881889763779528	\\
1.59593754802461	0.889763779527559	\\
1.59975618959618	0.897637795275591	\\
1.62396091012077	0.905511811023622	\\
1.63091356521893	0.913385826771654	\\
1.65396071714646	0.921259842519685	\\
1.74738024875709	0.929133858267717	\\
1.75062255312453	0.937007874015748	\\
1.79753781673795	0.94488188976378	\\
1.95769445725239	0.952755905511811	\\
1.98531226073519	0.960629921259843	\\
2.11076445620688	0.968503937007874	\\
2.17810964012715	0.976377952755906	\\
2.31186036321789	0.984251968503937	\\
2.47225071974494	0.992125984251969	\\
999	1	\\
};
\addlegendentry{$\delta1p4$}

\addplot [color=cyan,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
0.002141151149831756 0.007874015748031496\\
0.006244633515310735 0.015748031496062992\\
0.008902568822172776 0.023622047244094488\\
0.011716676153283222 0.031496062992125984\\
0.015037740319922404 0.03937007874015748\\
0.020292789274750245 0.047244094488188976\\
0.025592112157167713 0.05511811023622047\\
0.03141887796937553 0.06299212598425197\\
0.03193460413947663 0.07086614173228346\\
0.03251855391505606 0.07874015748031496\\
0.03729699844338945 0.08661417322834646\\
0.0400900177492693 0.09448818897637795\\
0.04361418234317862 0.10236220472440945\\
0.0446680896382562 0.11023622047244094\\
0.04474416981986836 0.11811023622047244\\
0.047036426127522304 0.12598425196850394\\
0.059596801181828585 0.13385826771653545\\
0.062322126119552006 0.14173228346456693\\
0.07343669490501915 0.14960629921259844\\
0.07573879603680694 0.15748031496062992\\
0.0813943307816336 0.16535433070866143\\
0.08209169541699372 0.1732283464566929\\
0.08482046755795397 0.18110236220472442\\
0.09951004140361325 0.1889763779527559\\
0.11347540497016137 0.1968503937007874\\
0.119653606069486 0.2047244094488189\\
0.12059467874973731 0.2125984251968504\\
0.1300957175627129 0.2204724409448819\\
0.13455595483692234 0.2283464566929134\\
0.1487695647706984 0.23622047244094488\\
0.1518352583431362 0.2440944881889764\\
0.15238681775178442 0.25196850393700787\\
0.17405139384904694 0.25984251968503935\\
0.17437412569388816 0.2677165354330709\\
0.19850813793434693 0.2755905511811024\\
0.2371761155683672 0.28346456692913385\\
0.24400909707688087 0.29133858267716534\\
0.2524476173961889 0.2992125984251969\\
0.2548798662840161 0.30708661417322836\\
0.2662441287098087 0.31496062992125984\\
0.27081786588510004 0.3228346456692913\\
0.2738770835150151 0.33070866141732286\\
0.27782731449272324 0.33858267716535434\\
0.2831015639587198 0.3464566929133858\\
0.28669517450434795 0.3543307086614173\\
0.28993526766052524 0.36220472440944884\\
0.3004102327471071 0.3700787401574803\\
0.30549882298107706 0.3779527559055118\\
0.31292604306682786 0.3858267716535433\\
0.31994082017855824 0.3937007874015748\\
0.32121939017907514 0.4015748031496063\\
0.3216646411766448 0.4094488188976378\\
0.32379215674324635 0.41732283464566927\\
0.339763261431898 0.4251968503937008\\
0.34018817624240977 0.4330708661417323\\
0.3587819565657219 0.4409448818897638\\
0.37018283052041634 0.44881889763779526\\
0.38012567261671104 0.4566929133858268\\
0.3818575914937054 0.4645669291338583\\
0.3980254092930946 0.47244094488188976\\
0.3986992129311428 0.48031496062992124\\
0.4142692259917151 0.4881889763779528\\
0.4185770426953113 0.49606299212598426\\
0.4299186833250624 0.5039370078740157\\
0.44544574324675723 0.5118110236220472\\
0.4459269474268154 0.5196850393700787\\
0.4533020313561369 0.5275590551181102\\
0.4541090354264762 0.5354330708661418\\
0.46941789713663545 0.5433070866141733\\
0.4724760249008305 0.5511811023622047\\
0.4891064272072554 0.5590551181102362\\
0.5006344960254924 0.5669291338582677\\
0.5034069705214431 0.5748031496062992\\
0.5115100188927422 0.5826771653543307\\
0.5191524635015535 0.5905511811023622\\
0.5214950297047287 0.5984251968503937\\
0.5308067268765624 0.6062992125984252\\
0.5329604579461261 0.6141732283464567\\
0.542909197340594 0.6220472440944882\\
0.5454457520731905 0.6299212598425197\\
0.5474608517337519 0.6377952755905512\\
0.547925752659463 0.6456692913385826\\
0.5531123695202494 0.6535433070866141\\
0.5914840990443175 0.6614173228346457\\
0.593912512412929 0.6692913385826772\\
0.5986566398176212 0.6771653543307087\\
0.6000449610287877 0.6850393700787402\\
0.6185386767969858 0.6929133858267716\\
0.6424683528299463 0.7007874015748031\\
0.667223797221431 0.7086614173228346\\
0.6710413875069071 0.7165354330708661\\
0.7181281144489524 0.7244094488188977\\
0.7591442889668151 0.7322834645669292\\
0.7673874619105815 0.7401574803149606\\
0.7783818407442352 0.7480314960629921\\
0.7857887686255395 0.7559055118110236\\
0.7965740086388727 0.7637795275590551\\
0.7976652754963361 0.7716535433070866\\
0.9402720242175108 0.7795275590551181\\
0.964514678586694 0.7874015748031497\\
0.9721254153913468 0.7952755905511811\\
1.0302166749501858 0.8031496062992126\\
1.0416204586966644 0.8110236220472441\\
1.0863310720657138 0.8188976377952756\\
1.0887971358750916 0.8267716535433071\\
1.1797059608584435 0.8346456692913385\\
1.2360850726569848 0.84251968503937\\
1.3157140995088903 0.8503937007874016\\
1.332245093392045 0.8582677165354331\\
2.4256332099355578 0.8661417322834646\\
2.6757895570455776 0.8740157480314961\\
2.7411487188004218 0.8818897637795275\\
2.9935673784431995 0.889763779527559\\
3.3406225020546536 0.8976377952755905\\
3.3898891579881267 0.905511811023622\\
3.4791371467727297 0.9133858267716536\\
3.7251973118611477 0.9212598425196851\\
3.8584709344982544 0.9291338582677166\\
4.07344229298897 0.937007874015748\\
4.646080909579191 0.9448818897637795\\
4.812135895732425 0.952755905511811\\
5.11991788075929 0.9606299212598425\\
5.274829458467839 0.968503937007874\\
6.145448297309133 0.9763779527559056\\
6.815263154311762 0.984251968503937\\
7.288095124721682 0.9921259842519685\\
7.492064801355152 1.0\\
};
\addlegendentry{$\delta1p5$}

\addplot [color=black,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0	0	\\
0.0335305553331041	0.0078740157480315	\\
0.0430582714576159	0.015748031496063	\\
0.0514980416957851	0.0236220472440945	\\
0.0570119016847759	0.031496062992126	\\
0.0584929853054468	0.0393700787401575	\\
0.0645790922546401	0.047244094488189	\\
0.112236420206025	0.0551181102362205	\\
0.171200796928587	0.062992125984252	\\
0.172289321518478	0.0708661417322835	\\
0.176847452706549	0.078740157480315	\\
0.181314123625912	0.0866141732283465	\\
0.187154695793892	0.094488188976378	\\
0.198753042520847	0.102362204724409	\\
0.224305898327122	0.110236220472441	\\
0.231644908566369	0.118110236220472	\\
0.255163598210777	0.125984251968504	\\
0.262977353991522	0.133858267716535	\\
0.269839697611405	0.141732283464567	\\
0.27113507301807	0.149606299212598	\\
0.276614764275257	0.15748031496063	\\
0.287512103293708	0.165354330708661	\\
0.316179831159291	0.173228346456693	\\
0.321445367404281	0.181102362204724	\\
0.325681187887271	0.188976377952756	\\
0.338019232489711	0.196850393700787	\\
0.340431480661406	0.204724409448819	\\
0.348865312212948	0.21259842519685	\\
0.35096162490481	0.220472440944882	\\
0.392491381281053	0.228346456692913	\\
0.436167435727904	0.236220472440945	\\
0.445588747902805	0.244094488188976	\\
0.455601807127333	0.251968503937008	\\
0.467909319928182	0.259842519685039	\\
0.471856319139558	0.267716535433071	\\
0.49408604978647	0.275590551181102	\\
0.501776716199355	0.283464566929134	\\
0.506085009329937	0.291338582677165	\\
0.512134596026122	0.299212598425197	\\
0.518452077025247	0.307086614173228	\\
0.522855030709731	0.31496062992126	\\
0.541855565420255	0.322834645669291	\\
0.545582910918767	0.330708661417323	\\
0.565419031173977	0.338582677165354	\\
0.569216752565608	0.346456692913386	\\
0.57201240044743	0.354330708661417	\\
0.572486419680144	0.362204724409449	\\
0.57878348131148	0.37007874015748	\\
0.626550556440732	0.377952755905512	\\
0.632617844212616	0.385826771653543	\\
0.650777638484738	0.393700787401575	\\
0.668089416461432	0.401574803149606	\\
0.688420598585041	0.409448818897638	\\
0.716545280781643	0.417322834645669	\\
0.725889044723639	0.425196850393701	\\
0.734587563024692	0.433070866141732	\\
0.7956027000628	0.440944881889764	\\
0.838861455003204	0.448818897637795	\\
0.874630928658189	0.456692913385827	\\
0.890416640761681	0.464566929133858	\\
0.924721329140087	0.47244094488189	\\
0.936695056626709	0.480314960629921	\\
0.939291823976901	0.488188976377953	\\
0.942530559733291	0.496062992125984	\\
0.964192384292147	0.503937007874016	\\
0.975620504584156	0.511811023622047	\\
0.995014451108542	0.519685039370079	\\
1.00844994419541	0.52755905511811	\\
1.0266409508193	0.535433070866142	\\
1.02722072193742	0.543307086614173	\\
1.05094939099805	0.551181102362205	\\
1.07039773131951	0.559055118110236	\\
1.08553273388849	0.566929133858268	\\
1.09822338448441	0.574803149606299	\\
1.14787523025091	0.582677165354331	\\
1.17093301141637	0.590551181102362	\\
1.20395743389692	0.598425196850394	\\
1.23619211851125	0.606299212598425	\\
1.26657963450491	0.614173228346457	\\
1.27431327969839	0.622047244094488	\\
1.29773317753568	0.62992125984252	\\
1.30304177044991	0.637795275590551	\\
1.32490445098992	0.645669291338583	\\
1.32687173567978	0.653543307086614	\\
1.36929143192776	0.661417322834646	\\
1.36932784349527	0.669291338582677	\\
1.38035677140285	0.677165354330709	\\
1.46020712731866	0.68503937007874	\\
1.49408175041096	0.692913385826772	\\
1.49650299403958	0.700787401574803	\\
1.57252313850546	0.708661417322835	\\
1.60314912132154	0.716535433070866	\\
1.61023539862037	0.724409448818898	\\
1.61772742354113	0.732283464566929	\\
1.67545307340751	0.740157480314961	\\
1.725400185637	0.748031496062992	\\
1.73985404462874	0.755905511811024	\\
1.78628110526345	0.763779527559055	\\
1.87652570336362	0.771653543307087	\\
1.91202903898932	0.779527559055118	\\
1.92191606226638	0.78740157480315	\\
1.98222613311509	0.795275590551181	\\
2.17008998923553	0.803149606299213	\\
2.20660679943766	0.811023622047244	\\
2.28758861117297	0.818897637795276	\\
2.4451566859689	0.826771653543307	\\
2.55429648405788	0.834645669291339	\\
2.61655643780819	0.84251968503937	\\
2.69382238739558	0.850393700787402	\\
3.37397231984032	0.858267716535433	\\
99	0.866141732283465	\\
100	0.874015748031496	\\
101	0.881889763779528	\\
102	0.889763779527559	\\
103	0.897637795275591	\\
104	0.905511811023622	\\
105	0.913385826771654	\\
106	0.921259842519685	\\
107	0.929133858267717	\\
108	0.937007874015748	\\
109	0.94488188976378	\\
110	0.952755905511811	\\
111	0.960629921259843	\\
112	0.968503937007874	\\
113	0.976377952755906	\\
114	0.984251968503937	\\
115	0.992125984251969	\\
116	1	\\
};
\addlegendentry{$LAAA$}

\legend{}

\end{axis}

==> Plot/real_t_line.tex <==
\begin{axis}[%
%xmode=log,
width=0.16\columnwidth,
height=0.10\columnwidth,
at={(1.05in,0.389in)},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black}},
xlabel={Line err ($^{\circ}$)},
ymin=0,
ymax=1,
ytick={0,0.5,1},
%ytick={0,10000},
%xtick={1e-6,1e-15},
%ytick={0,10000},
ymode=normal,
xlabel style={yshift=0.07in},
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=red,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
};
\addlegendentry{$d1p4P$}

\addplot [color=green,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
0.3295212968995868 0.02\\
0.9076458909204652 0.04\\
1.1495303236570258 0.06\\
1.7911359998373684 0.08\\
1.9955274069531552 0.1\\
2.097359841539702 0.12\\
2.8970297935584677 0.14\\
3.815996882189064 0.16\\
4.313354376958467 0.18\\
4.465707257961296 0.2\\
4.9295968400669015 0.22\\
4.9647169176338615 0.24\\
5.7665040384765796 0.26\\
5.847657044805466 0.28\\
5.932215952984777 0.3\\
6.153784788804715 0.32\\
6.158388890045988 0.34\\
6.339915691684399 0.36\\
6.457720350343573 0.38\\
6.556377297635943 0.4\\
7.297180435086145 0.42\\
7.980716220519769 0.44\\
8.252226568660797 0.46\\
8.73864694814132 0.48\\
8.771805908370963 0.5\\
8.862874811938163 0.52\\
9.225175599651623 0.54\\
10.600704022368626 0.56\\
11.196304760784315 0.58\\
13.704626524682192 0.6\\
13.89110113511021 0.62\\
14.221346163167285 0.64\\
15.494722470936459 0.66\\
19.6009426625411 0.68\\
20.56598456623468 0.7\\
20.90686464714254 0.72\\
22.7148689434004 0.74\\
26.8398393440849 0.76\\
27.745833608390534 0.78\\
30.302946420278985 0.8\\
31.603030124240956 0.82\\
31.82854944067867 0.84\\
31.95282130193604 0.86\\
36.157178163985805 0.88\\
36.73010376130394 0.9\\
37.455357485136325 0.92\\
61.767673598602386 0.94\\
74.57495079142713 0.96\\
78.62184710833796 0.98\\
89.18466381565777 1.0\\
};
\addlegendentry{$d1p3P$}

\addplot [color=blue,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
0.17836151219389282 0.02\\
0.3101615497233222 0.04\\
0.5776045101221428 0.06\\
0.787242390494117 0.08\\
0.9698016746532293 0.1\\
1.0153337885957723 0.12\\
1.0181843828056603 0.14\\
1.040695819522408 0.16\\
1.0832856329219827 0.18\\
1.1177975042862192 0.2\\
1.1412712013751216 0.22\\
1.196716038849593 0.24\\
1.202100710551431 0.26\\
1.471365079111312 0.28\\
1.5192484128640529 0.3\\
1.6089088623591 0.32\\
1.7349981706069946 0.34\\
1.7439441635263095 0.36\\
1.754598824812011 0.38\\
1.778980210426908 0.4\\
1.8545538753020676 0.42\\
2.1857751883381726 0.44\\
2.2115649269237982 0.46\\
2.2952147177340017 0.48\\
2.38884619725713 0.5\\
2.3952126013357864 0.52\\
2.4019668441961777 0.54\\
2.542353329084165 0.56\\
2.5975419500114354 0.58\\
2.658850772455658 0.6\\
2.703805966301028 0.62\\
2.9622862464186683 0.64\\
3.1944922873163852 0.66\\
3.2968424898712327 0.68\\
3.742094124158826 0.7\\
3.820608227597055 0.72\\
3.8234276859766054 0.74\\
4.229745631184244 0.76\\
4.316918077985689 0.78\\
4.36289542850782 0.8\\
4.505687278155941 0.82\\
4.626452180574362 0.84\\
4.925622336311773 0.86\\
5.163529155263515 0.88\\
6.080110489259371 0.9\\
6.693461559965952 0.92\\
6.737549270556088 0.94\\
7.989623835693146 0.96\\
18.295438321417812 0.98\\
61.898051227453294 1.0\\
};
\addlegendentry{$d1p3PC$}

\addplot [color=magenta,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
0 0\\
0.19638399497494355 0.02\\
0.35021944113014847 0.04\\
0.3682682779019611 0.06\\
0.43043094078774646 0.08\\
0.6184666223462912 0.1\\
0.6753784747933315 0.12\\
0.7121790331201365 0.14\\
0.7236598149218738 0.16\\
1.0313844597493833 0.18\\
1.355106445160571 0.2\\
1.4928753477758563 0.22\\
1.564428519290277 0.24\\
1.7171365472409095 0.26\\
1.9002300701313366 0.28\\
2.0214552528854934 0.3\\
2.2236125631450125 0.32\\
2.2978005918550717 0.34\\
2.3460675671736095 0.36\\
2.3543824993797053 0.38\\
2.4166739391137635 0.4\\
2.563687861752916 0.42\\
2.6436336516744636 0.44\\
2.7598994119907485 0.46\\
2.9739595810660853 0.48\\
3.0671210137243303 0.5\\
3.153555216052399 0.52\\
3.166323556302731 0.54\\
3.2411405920509266 0.56\\
3.27242120019626 0.58\\
3.392921930283068 0.6\\
3.5264213605234005 0.62\\
3.63291346107291 0.64\\
3.8346495721672738 0.66\\
4.0743750993625705 0.68\\
4.483423704943584 0.7\\
4.55795528354129 0.72\\
5.093957183570192 0.74\\
5.119190140958661 0.76\\
5.1877108320799135 0.78\\
7.084498823224963 0.8\\
7.1447891153459695 0.82\\
7.167098495121868 0.84\\
8.55437432959349 0.86\\
9.461099646949453 0.88\\
9.769230766446618 0.9\\
9.982417092336972 0.92\\
10.015344487688958 0.94\\
15.903628679458246 0.96\\
18.065219594330824 0.98\\
45.41301820383617 1.0\\
};
\addlegendentry{$d1p2PC$}

\legend{}

\end{axis}

\input{Plot/real_r_axis.tex}

==> Plot/stability_r_angle.tex <==
\begin{axis}[%
xmode=log,
width=0.16\columnwidth,
height=0.10\columnwidth,
at={(3.0in,0.389in)},
scale only axis,
xmin=1e-13,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={Norm err (rel.)},
ymin=0,
ymax=30000,
%ytick={0,10000},
xtick={1e-6,1e-0},
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=VeryPink,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.31826e-20 0 \\
2.29087e-20 0 \\
3.98107e-20 0 \\
6.91831e-20 0 \\
1.20226e-19 0 \\
2.0893e-19 0 \\
3.63078e-19 0 \\
6.30957e-19 8 \\
1.09648e-18 0 \\
1.90546e-18 0 \\
3.31131e-18 0 \\
5.7544e-18 0 \\
1e-17 0 \\
1.7378e-17 0 \\
3.01995e-17 0 \\
5.24807e-17 0 \\
9.12011e-17 0 \\
1.58489e-16 0 \\
2.75423e-16 0 \\
4.7863e-16 0 \\
8.31764e-16 0 \\
1.44544e-15 0 \\
2.51189e-15 0 \\
4.36516e-15 0 \\
7.58578e-15 14 \\
1.31826e-14 26 \\
2.29087e-14 25 \\
3.98107e-14 61 \\
6.91831e-14 103 \\
1.20226e-13 174 \\
2.0893e-13 297 \\
3.63078e-13 487 \\
6.30957e-13 740 \\
1.09648e-12 1137 \\
1.90546e-12 1532 \\
3.31131e-12 2015 \\
5.7544e-12 2542 \\
1e-11 2858 \\
1.7378e-11 3175 \\
3.01995e-11 3517 \\
5.24807e-11 3704 \\
9.12011e-11 3616 \\
1.58489e-10 3783 \\
2.75423e-10 3866 \\
4.7863e-10 3698 \\
8.31764e-10 3760 \\
1.44544e-09 3781 \\
2.51189e-09 3778 \\
4.36516e-09 3704 \\
7.58578e-09 3765 \\
1.31826e-08 3828 \\
2.29087e-08 3835 \\
3.98107e-08 3936 \\
6.91831e-08 3791 \\
1.20226e-07 3858 \\
2.0893e-07 3567 \\
3.63078e-07 3060 \\
6.30957e-07 2636 \\
1.09648e-06 2204 \\
1.90546e-06 1611 \\
3.31131e-06 1116 \\
5.7544e-06 785 \\
1e-05 525 \\
1.7378e-05 323 \\
3.01995e-05 204 \\
5.24807e-05 138 \\
9.12011e-05 78 \\
0.000158489 50 \\
0.000275423 50 \\
0.00047863 20 \\
0.000831764 10 \\
0.00144544 11 \\
0.00251189 4 \\
0.00436516 4 \\
0.00758578 3 \\
0.0131826 1 \\
0.0229087 3 \\
0.0398107 5 \\
0.0691831 9 \\
0.120226 8 \\
0.20893 10 \\
0.363078 32 \\
0.630957 38 \\
1.09648 56 \\
1.90546 82 \\
3.31131 120 \\
5.7544 197 \\
10 283 \\
17.378 341 \\
30.1995 442 \\
52.4807 906 \\
91.2011 4451 \\
158.489 972 \\
275.423 159 \\
478.63 52 \\
831.764 11 \\
1445.44 5 \\
2511.89 2 \\
4365.16 0 \\
7585.78 2 \\
};
\addlegendentry{$\delta1p3$}

\addplot [color=brown,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.31826e-20 0 \\
2.29087e-20 0 \\
3.98107e-20 0 \\
6.91831e-20 0 \\
1.20226e-19 0 \\
2.0893e-19 0 \\
3.63078e-19 0 \\
6.30957e-19 2 \\
1.09648e-18 0 \\
1.90546e-18 0 \\
3.31131e-18 0 \\
5.7544e-18 0 \\
1e-17 0 \\
1.7378e-17 0 \\
3.01995e-17 0 \\
5.24807e-17 0 \\
9.12011e-17 0 \\
1.58489e-16 0 \\
2.75423e-16 0 \\
4.7863e-16 0 \\
8.31764e-16 0 \\
1.44544e-15 0 \\
2.51189e-15 0 \\
4.36516e-15 0 \\
7.58578e-15 2 \\
1.31826e-14 8 \\
2.29087e-14 7 \\
3.98107e-14 15 \\
6.91831e-14 35 \\
1.20226e-13 45 \\
2.0893e-13 95 \\
3.63078e-13 141 \\
6.30957e-13 249 \\
1.09648e-12 405 \\
1.90546e-12 636 \\
3.31131e-12 876 \\
5.7544e-12 1283 \\
1e-11 1627 \\
1.7378e-11 2021 \\
3.01995e-11 2389 \\
5.24807e-11 2829 \\
9.12011e-11 3126 \\
1.58489e-10 3440 \\
2.75423e-10 3738 \\
4.7863e-10 3824 \\
8.31764e-10 4031 \\
1.44544e-09 3992 \\
2.51189e-09 4080 \\
4.36516e-09 4159 \\
7.58578e-09 4181 \\
1.31826e-08 4256 \\
2.29087e-08 4394 \\
3.98107e-08 4457 \\
6.91831e-08 4445 \\
1.20226e-07 4385 \\
2.0893e-07 4205 \\
3.63078e-07 3845 \\
6.30957e-07 3512 \\
1.09648e-06 3057 \\
1.90546e-06 2486 \\
3.31131e-06 1772 \\
5.7544e-06 1241 \\
1e-05 833 \\
1.7378e-05 530 \\
3.01995e-05 361 \\
5.24807e-05 193 \\
9.12011e-05 175 \\
0.000158489 85 \\
0.000275423 57 \\
0.00047863 42 \\
0.000831764 21 \\
0.00144544 19 \\
0.00251189 6 \\
0.00436516 1 \\
0.00758578 1 \\
0.0131826 2 \\
0.0229087 4 \\
0.0398107 5 \\
0.0691831 5 \\
0.120226 11 \\
0.20893 19 \\
0.363078 32 \\
0.630957 69 \\
1.09648 81 \\
1.90546 146 \\
3.31131 185 \\
5.7544 287 \\
10 404 \\
17.378 568 \\
30.1995 681 \\
52.4807 1087 \\
91.2011 3571 \\
158.489 1126 \\
275.423 86 \\
478.63 8 \\
831.764 0 \\
1445.44 0 \\
2511.89 2 \\
4365.16 1 \\
7585.78 5 \\
};
\addlegendentry{$\delta1p4$}

\addplot [color=cyan,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.31826e-20 0 \\
2.29087e-20 0 \\
3.98107e-20 0 \\
6.91831e-20 0 \\
1.20226e-19 0 \\
2.0893e-19 0 \\
3.63078e-19 0 \\
6.30957e-19 0 \\
1.09648e-18 0 \\
1.90546e-18 0 \\
3.31131e-18 0 \\
5.7544e-18 0 \\
1e-17 0 \\
1.7378e-17 0 \\
3.01995e-17 0 \\
5.24807e-17 0 \\
9.12011e-17 0 \\
1.58489e-16 0 \\
2.75423e-16 0 \\
4.7863e-16 0 \\
8.31764e-16 0 \\
1.44544e-15 2 \\
2.51189e-15 4 \\
4.36516e-15 3 \\
7.58578e-15 4 \\
1.31826e-14 12 \\
2.29087e-14 28 \\
3.98107e-14 44 \\
6.91831e-14 56 \\
1.20226e-13 98 \\
2.0893e-13 189 \\
3.63078e-13 269 \\
6.30957e-13 430 \\
1.09648e-12 676 \\
1.90546e-12 915 \\
3.31131e-12 1388 \\
5.7544e-12 1921 \\
1e-11 2508 \\
1.7378e-11 3267 \\
3.01995e-11 3970 \\
5.24807e-11 4650 \\
9.12011e-11 5369 \\
1.58489e-10 5480 \\
2.75423e-10 5745 \\
4.7863e-10 6108 \\
8.31764e-10 6058 \\
1.44544e-09 6063 \\
2.51189e-09 6192 \\
4.36516e-09 5883 \\
7.58578e-09 5928 \\
1.31826e-08 5603 \\
2.29087e-08 4843 \\
3.98107e-08 3756 \\
6.91831e-08 2322 \\
1.20226e-07 1250 \\
2.0893e-07 906 \\
3.63078e-07 599 \\
6.30957e-07 391 \\
1.09648e-06 307 \\
1.90546e-06 212 \\
3.31131e-06 117 \\
5.7544e-06 91 \\
1e-05 57 \\
1.7378e-05 23 \\
3.01995e-05 9 \\
5.24807e-05 3 \\
9.12011e-05 4 \\
0.000158489 1 \\
0.000275423 3 \\
0.00047863 2 \\
0.000831764 11 \\
0.00144544 17 \\
0.00251189 29 \\
0.00436516 43 \\
0.00758578 68 \\
0.0131826 125 \\
0.0229087 221 \\
0.0398107 372 \\
0.0691831 564 \\
0.120226 957 \\
0.20893 1241 \\
0.363078 886 \\
0.630957 445 \\
1.09648 261 \\
1.90546 256 \\
3.31131 93 \\
5.7544 275 \\
10 260 \\
17.378 88 \\
30.1995 15 \\
52.4807 6 \\
91.2011 3 \\
158.489 1 \\
275.423 1 \\
478.63 0 \\
831.764 2 \\
1445.44 1 \\
2511.89 0 \\
4365.16 0 \\
7585.78 0 \\
};
\addlegendentry{$\delta1p5$}

\addplot [color=black,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.31826e-20 0 \\
2.29087e-20 0 \\
3.98107e-20 0 \\
6.91831e-20 0 \\
1.20226e-19 0 \\
2.0893e-19 0 \\
3.63078e-19 0 \\
6.30957e-19 0 \\
1.09648e-18 0 \\
1.90546e-18 0 \\
3.31131e-18 0 \\
5.7544e-18 0 \\
1e-17 0 \\
1.7378e-17 0 \\
3.01995e-17 0 \\
5.24807e-17 0 \\
9.12011e-17 0 \\
1.58489e-16 0 \\
2.75423e-16 0 \\
4.7863e-16 0 \\
8.31764e-16 0 \\
1.44544e-15 0 \\
2.51189e-15 0 \\
4.36516e-15 0 \\
7.58578e-15 0 \\
1.31826e-14 0 \\
2.29087e-14 0 \\
3.98107e-14 0 \\
6.91831e-14 0 \\
1.20226e-13 0 \\
2.0893e-13 0 \\
3.63078e-13 0 \\
6.30957e-13 0 \\
1.09648e-12 0 \\
1.90546e-12 0 \\
3.31131e-12 0 \\
5.7544e-12 0 \\
1e-11 0 \\
1.7378e-11 0 \\
3.01995e-11 0 \\
5.24807e-11 0 \\
9.12011e-11 0 \\
1.58489e-10 0 \\
2.75423e-10 0 \\
4.7863e-10 0 \\
8.31764e-10 0 \\
1.44544e-09 0 \\
2.51189e-09 0 \\
4.36516e-09 0 \\
7.58578e-09 0 \\
1.31826e-08 0 \\
2.29087e-08 0 \\
3.98107e-08 0 \\
6.91831e-08 0 \\
1.20226e-07 0 \\
2.0893e-07 0 \\
3.63078e-07 0 \\
6.30957e-07 0 \\
1.09648e-06 0 \\
1.90546e-06 0 \\
3.31131e-06 0 \\
5.7544e-06 0 \\
1e-05 0 \\
1.7378e-05 0 \\
3.01995e-05 0 \\
5.24807e-05 0 \\
9.12011e-05 0 \\
0.000158489 1 \\
0.000275423 1 \\
0.00047863 0 \\
0.000831764 0 \\
0.00144544 3 \\
0.00251189 2 \\
0.00436516 9 \\
0.00758578 9 \\
0.0131826 10 \\
0.0229087 29 \\
0.0398107 40 \\
0.0691831 89 \\
0.120226 133 \\
0.20893 259 \\
0.363078 433 \\
0.630957 699 \\
1.09648 1322 \\
1.90546 2260 \\
3.31131 3808 \\
5.7544 6181 \\
10 9017 \\
17.378 11966 \\
30.1995 14821 \\
52.4807 20388 \\
91.2011 19125 \\
158.489 7321 \\
275.423 1746 \\
478.63 286 \\
831.764 30 \\
1445.44 7 \\
2511.89 0 \\
4365.16 3 \\
7585.78 2 \\
};
\addlegendentry{$LAAA$}

\legend{}

\end{axis}

==> Plot/stability_t_line.tex <==
\begin{axis}[%
xmode=log,
width=0.16\columnwidth,
height=0.10\columnwidth,
at={(1.0in,0.389in)},
scale only axis,
xmin=1e-10,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={Line err ($^\circ$)},
ymin=0,
ymax=30000,
%ytick={0,10000,20000},
xtick={1e-6,1e0},
ymode=normal,
yminorticks=true,
axis lines = left,
axis background/.style={fill=white},
title style={font=\bfseries},
%ylabel style={yshift=-0.15in},
%ylabel={Frequency},
legend style={at={(1,1.3)}, anchor=south, legend cell align=left, align=left, draw=white!15!black, font=\normalsize,nodes={scale=1.0, transform shape}},
legend columns=6
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addplot [color=red,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.28825e-20 0 \\
2.13796e-20 0 \\
3.54813e-20 0 \\
5.88844e-20 0 \\
9.77237e-20 0 \\
1.62181e-19 0 \\
2.69153e-19 0 \\
4.46684e-19 0 \\
7.4131e-19 0 \\
1.23027e-18 0 \\
2.04174e-18 0 \\
3.38844e-18 0 \\
5.62341e-18 0 \\
9.33254e-18 0 \\
1.54882e-17 0 \\
2.5704e-17 0 \\
4.2658e-17 0 \\
7.07946e-17 0 \\
1.1749e-16 0 \\
1.94984e-16 0 \\
3.23594e-16 0 \\
5.37032e-16 0 \\
8.91251e-16 0 \\
1.47911e-15 0 \\
2.45471e-15 0 \\
4.0738e-15 0 \\
6.76083e-15 0 \\
1.12202e-14 0 \\
1.86209e-14 0 \\
3.0903e-14 0 \\
5.12861e-14 0 \\
8.51138e-14 0 \\
1.41254e-13 0 \\
2.34423e-13 0 \\
3.89045e-13 0 \\
6.45654e-13 0 \\
1.07152e-12 0 \\
1.77828e-12 0 \\
2.95121e-12 0 \\
4.89779e-12 0 \\
8.12831e-12 0 \\
1.34896e-11 0 \\
2.23872e-11 0 \\
3.71535e-11 0 \\
6.16595e-11 0 \\
1.02329e-10 0 \\
1.69824e-10 0 \\
2.81838e-10 0 \\
4.67735e-10 0 \\
7.76247e-10 0 \\
1.28825e-09 0 \\
2.13796e-09 0 \\
3.54813e-09 1 \\
5.88844e-09 8 \\
9.77237e-09 19 \\
1.62181e-08 47 \\
2.69153e-08 147 \\
4.46684e-08 393 \\
7.4131e-08 1045 \\
1.23027e-07 2890 \\
2.04174e-07 7917 \\
3.38844e-07 20323 \\
5.62341e-07 34521 \\
9.33254e-07 19077 \\
1.54882e-06 2296 \\
2.5704e-06 766 \\
4.2658e-06 491 \\
7.07946e-06 332 \\
1.1749e-05 232 \\
1.94984e-05 169 \\
3.23594e-05 88 \\
5.37032e-05 68 \\
8.91251e-05 50 \\
0.000147911 26 \\
0.000245471 12 \\
0.00040738 13 \\
0.000676083 4 \\
0.00112202 2 \\
0.00186209 6 \\
0.0030903 3 \\
0.00512861 1 \\
0.00851138 0 \\
0.0141254 1 \\
0.0234423 3 \\
0.0389045 6 \\
0.0645654 3 \\
0.107152 13 \\
0.177828 24 \\
0.295121 41 \\
0.489779 41 \\
0.812831 67 \\
1.34896 121 \\
2.23872 143 \\
3.71535 222 \\
6.16595 314 \\
10.2329 477 \\
16.9824 793 \\
28.1838 1333 \\
46.7735 2478 \\
77.6247 2973 \\
};
\addlegendentry{$d1p2P$}

\addplot [color=green,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.28825e-20 0 \\
2.13796e-20 0 \\
3.54813e-20 0 \\
5.88844e-20 0 \\
9.77237e-20 0 \\
1.62181e-19 0 \\
2.69153e-19 0 \\
4.46684e-19 0 \\
7.4131e-19 0 \\
1.23027e-18 0 \\
2.04174e-18 0 \\
3.38844e-18 0 \\
5.62341e-18 0 \\
9.33254e-18 0 \\
1.54882e-17 0 \\
2.5704e-17 0 \\
4.2658e-17 0 \\
7.07946e-17 0 \\
1.1749e-16 0 \\
1.94984e-16 0 \\
3.23594e-16 0 \\
5.37032e-16 0 \\
8.91251e-16 0 \\
1.47911e-15 0 \\
2.45471e-15 0 \\
4.0738e-15 0 \\
6.76083e-15 0 \\
1.12202e-14 0 \\
1.86209e-14 0 \\
3.0903e-14 0 \\
5.12861e-14 0 \\
8.51138e-14 0 \\
1.41254e-13 0 \\
2.34423e-13 0 \\
3.89045e-13 0 \\
6.45654e-13 0 \\
1.07152e-12 0 \\
1.77828e-12 0 \\
2.95121e-12 0 \\
4.89779e-12 0 \\
8.12831e-12 0 \\
1.34896e-11 0 \\
2.23872e-11 0 \\
3.71535e-11 0 \\
6.16595e-11 0 \\
1.02329e-10 0 \\
1.69824e-10 0 \\
2.81838e-10 0 \\
4.67735e-10 0 \\
7.76247e-10 0 \\
1.28825e-09 0 \\
2.13796e-09 1 \\
3.54813e-09 1 \\
5.88844e-09 6 \\
9.77237e-09 22 \\
1.62181e-08 54 \\
2.69153e-08 154 \\
4.46684e-08 407 \\
7.4131e-08 1122 \\
1.23027e-07 3162 \\
2.04174e-07 8296 \\
3.38844e-07 21408 \\
5.62341e-07 36036 \\
9.33254e-07 18467 \\
1.54882e-06 954 \\
2.5704e-06 35 \\
4.2658e-06 32 \\
7.07946e-06 24 \\
1.1749e-05 13 \\
1.94984e-05 13 \\
3.23594e-05 24 \\
5.37032e-05 20 \\
8.91251e-05 21 \\
0.000147911 30 \\
0.000245471 39 \\
0.00040738 46 \\
0.000676083 51 \\
0.00112202 47 \\
0.00186209 82 \\
0.0030903 79 \\
0.00512861 93 \\
0.00851138 116 \\
0.0141254 134 \\
0.0234423 162 \\
0.0389045 213 \\
0.0645654 218 \\
0.107152 230 \\
0.177828 254 \\
0.295121 226 \\
0.489779 223 \\
0.812831 202 \\
1.34896 203 \\
2.23872 177 \\
3.71535 176 \\
6.16595 208 \\
10.2329 243 \\
16.9824 459 \\
28.1838 954 \\
46.7735 1976 \\
77.6247 2887 \\
};
\addlegendentry{$d1p3P$}

\addplot [color=blue,line width=1.5pt, mark options={solid, blue}]
  table[row sep=crcr]{%
1.28825e-20 0 \\
2.13796e-20 0 \\
3.54813e-20 0 \\
5.88844e-20 0 \\
9.77237e-20 0 \\
1.62181e-19 0 \\
2.69153e-19 0 \\
4.46684e-19 2 \\
7.4131e-19 0 \\
1.23027e-18 0 \\
2.04174e-18 0 \\
3.38844e-18 0 \\
5.62341e-18 0 \\
9.33254e-18 0 \\
1.54882e-17 0 \\
2.5704e-17 0 \\
4.2658e-17 0 \\
7.07946e-17 0 \\
1.1749e-16 0 \\
1.94984e-16 0 \\
3.23594e-16 0 \\
5.37032e-16 0 \\
8.91251e-16 0 \\
1.47911e-15 0 \\
2.45471e-15 0 \\
4.0738e-15 0 \\
6.76083e-15 0 \\
1.12202e-14 0 \\
1.86209e-14 0 \\
3.0903e-14 0 \\
5.12861e-14 0 \\
8.51138e-14 0 \\
1.41254e-13 0 \\
2.34423e-13 0 \\
3.89045e-13 0 \\
6.45654e-13 0 \\
1.07152e-12 0 \\
1.77828e-12 0 \\
2.95121e-12 0 \\
4.89779e-12 0 \\
8.12831e-12 0 \\
1.34896e-11 0 \\
2.23872e-11 0 \\
3.71535e-11 0 \\
6.16595e-11 0 \\
1.02329e-10 0 \\
1.69824e-10 0 \\
2.81838e-10 0 \\
4.67735e-10 0 \\
7.76247e-10 0 \\
1.28825e-09 1 \\
2.13796e-09 1 \\
3.54813e-09 4 \\
5.88844e-09 8 \\
9.77237e-09 14 \\
1.62181e-08 39 \\
2.69153e-08 130 \\
4.46684e-08 344 \\
7.4131e-08 891 \\
1.23027e-07 2614 \\
2.04174e-07 6793 \\
3.38844e-07 17414 \\
5.62341e-07 29379 \\
9.33254e-07 15026 \\
1.54882e-06 791 \\
2.5704e-06 106 \\
4.2658e-06 95 \\
7.07946e-06 76 \\
1.1749e-05 56 \\
1.94984e-05 39 \\
3.23594e-05 25 \\
5.37032e-05 30 \\
8.91251e-05 20 \\
0.000147911 13 \\
0.000245471 13 \\
0.00040738 9 \\
0.000676083 16 \\
0.00112202 20 \\
0.00186209 44 \\
0.0030903 54 \\
0.00512861 73 \\
0.00851138 111 \\
0.0141254 170 \\
0.0234423 214 \\
0.0389045 242 \\
0.0645654 329 \\
0.107152 344 \\
0.177828 289 \\
0.295121 299 \\
0.489779 260 \\
0.812831 166 \\
1.34896 149 \\
2.23872 190 \\
3.71535 273 \\
6.16595 465 \\
10.2329 767 \\
16.9824 1497 \\
28.1838 3155 \\
46.7735 6781 \\
77.6247 10159 \\
};
\addlegendentry{$d1p3PC$}

\addplot [color=magenta,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.28825e-20 0 \\
2.13796e-20 0 \\
3.54813e-20 0 \\
5.88844e-20 0 \\
9.77237e-20 0 \\
1.62181e-19 0 \\
2.69153e-19 0 \\
4.46684e-19 0 \\
7.4131e-19 0 \\
1.23027e-18 0 \\
2.04174e-18 0 \\
3.38844e-18 0 \\
5.62341e-18 0 \\
9.33254e-18 0 \\
1.54882e-17 0 \\
2.5704e-17 0 \\
4.2658e-17 0 \\
7.07946e-17 0 \\
1.1749e-16 0 \\
1.94984e-16 0 \\
3.23594e-16 0 \\
5.37032e-16 0 \\
8.91251e-16 0 \\
1.47911e-15 0 \\
2.45471e-15 0 \\
4.0738e-15 0 \\
6.76083e-15 0 \\
1.12202e-14 0 \\
1.86209e-14 0 \\
3.0903e-14 0 \\
5.12861e-14 0 \\
8.51138e-14 0 \\
1.41254e-13 0 \\
2.34423e-13 0 \\
3.89045e-13 0 \\
6.45654e-13 0 \\
1.07152e-12 0 \\
1.77828e-12 0 \\
2.95121e-12 0 \\
4.89779e-12 0 \\
8.12831e-12 0 \\
1.34896e-11 0 \\
2.23872e-11 0 \\
3.71535e-11 0 \\
6.16595e-11 0 \\
1.02329e-10 0 \\
1.69824e-10 0 \\
2.81838e-10 0 \\
4.67735e-10 0 \\
7.76247e-10 0 \\
1.28825e-09 0 \\
2.13796e-09 0 \\
3.54813e-09 1 \\
5.88844e-09 7 \\
9.77237e-09 16 \\
1.62181e-08 29 \\
2.69153e-08 88 \\
4.46684e-08 287 \\
7.4131e-08 775 \\
1.23027e-07 2046 \\
2.04174e-07 5658 \\
3.38844e-07 14348 \\
5.62341e-07 23779 \\
9.33254e-07 12383 \\
1.54882e-06 674 \\
2.5704e-06 97 \\
4.2658e-06 65 \\
7.07946e-06 56 \\
1.1749e-05 36 \\
1.94984e-05 33 \\
3.23594e-05 21 \\
5.37032e-05 12 \\
8.91251e-05 11 \\
0.000147911 17 \\
0.000245471 4 \\
0.00040738 10 \\
0.000676083 12 \\
0.00112202 26 \\
0.00186209 32 \\
0.0030903 34 \\
0.00512861 50 \\
0.00851138 66 \\
0.0141254 100 \\
0.0234423 126 \\
0.0389045 152 \\
0.0645654 149 \\
0.107152 127 \\
0.177828 121 \\
0.295121 102 \\
0.489779 85 \\
0.812831 79 \\
1.34896 65 \\
2.23872 83 \\
3.71535 108 \\
6.16595 215 \\
10.2329 458 \\
16.9824 1136 \\
28.1838 4034 \\
46.7735 12322 \\
77.6247 19865 \\
};
\addlegendentry{$d1p2PC$}

\addplot [color=orange,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
};
\addlegendentry{$d2p6$}

\addplot [color=gray,line width=1.5pt, mark options={solid, red}]
  table[row sep=crcr]{%
1.334050268600027769e-20 0.000000000000000000e+00 \\
};
\addlegendentry{$d3p8$}

\legend{}


\end{axis}

\input{Plot/stability_r_axis}
